E-Waste-Bench: A Large-Scale Benchmark for Visual Triage of Data-Center Hardware

Retired data-center hardware can often be refurbished or resold, but triage demands more than object categories. A model must tell visually similar parts apart, judge condition under damage and occlusion, and read the printed part number. We audit nine public e-waste collections. They cover mostly consumer devices (only 10% of images are labeled as a data-center part), label neither condition nor printed text, and contain 42% exact or augmented duplicates. We introduce E-Waste-Bench, 328K photographs drawn from 762K deduplicated images and labeled for class (24 classes), granularity, condition and printed text. Images come from those collections and the web, where a recipe-based crawler works beside an agent built on an open-weight vision-language model. The agent vets new sources and reads sites the crawler cannot parse, and both are steered toward under-represented classes. Training labels are model-made, splits follow near-duplicate groups, and human annotators label a test set of nearly 10,000 images. We benchmark classification, condition, detection, text perception and cross-dataset transfer. On this test set, a ConvNeXt-T trained on E-Waste-Bench reaches 64.3% top-1, against 31.5% with the public collections alone. Near-duplicate leakage inflates top-1 by 3.0 points under model-made test labels but by less than 0.1 under human labels, so model-labeled benchmarks need group splits. Accuracy falls to 42.1% on marketplace and auction photographs, the closest proxy for hardware leaving service. Data and code will be released.

==> gold/tables/classification.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
\caption{Classification on the human-labeled test images, mean over seeds. Agreed: top-1 on the 782 images two annotators gave the same class. Named: top-1 on images given one of the 24 classes. None: recall on images marked none. Tail: accuracy on the third of the classes with the fewest training images, trained models only. Annotator: one annotator scored against another on doubly answered images. $^\dagger$Made the training class labels. Best in bold, annotator row aside. Higher is better. Full table: supplementary \cref{tab:cls_full}. Human labels.}
\label{tab:cls}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrr}
\toprule
model & top-1 & agreed & named & none & macro-F1 & tail \\
\midrule
\multicolumn{7}{c}{\textbf{Trained on the training set}} \\
\midrule
ResNet-50 & 63.5 & 75.1 & 71.6 & 33.3 & 60.0 & 56.4 \\
ConvNeXt-T & 64.3 & 76.9 & 72.2 & 34.9 & 60.6 & 57.6 \\
ConvNeXt-B & 65.0 & 77.1 & 73.0 & 35.2 & 61.1 & 57.9 \\
ViT-B/16 & 64.6 & 75.6 & 72.5 & 35.1 & 60.9 & \textbf{58.3} \\
EfficientNet-B3 & 64.5 & 75.8 & 72.0 & 36.5 & 60.2 & 56.9 \\
\midrule
\multicolumn{7}{c}{\textbf{Frozen features}} \\
\midrule
DINOv2-L linear & 64.0 & 75.6 & 70.9 & 38.2 & 59.6 & - \\
CLIP L/14 linear & 62.0 & 72.3 & 67.6 & 41.1 & 56.6 & - \\
CLIP B/32 linear & 62.0 & 73.0 & 67.4 & \textbf{42.0} & 56.7 & - \\
\midrule
\multicolumn{7}{c}{\textbf{Zero-shot}} \\
\midrule
CLIP L/14 zero-shot & 43.2 & 52.7 & 52.4 & 9.0 & 40.1 & - \\
CLIP B/32 zero-shot & 46.6 & 56.0 & 56.8 & 8.7 & 46.3 & - \\
Qwen3.5 zero-shot$^\dagger$ & \textbf{66.2} & \textbf{80.4} & \textbf{77.9} & 22.1 & \textbf{65.9} & - \\
Gemma~3 zero-shot & 59.8 & 73.3 & 70.6 & 19.2 & 59.4 & - \\
\midrule
\multicolumn{7}{c}{\textbf{Human annotators}} \\
\midrule
annotator vs. annotator & 74.0 & - & 76.8 & 62.3 & 69.0 & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> gold/tables/detection.tex <==
\begin{table}[t]
\centering
\small
\caption{Detection on the test images annotators gave one of the 24 classes. Found: a detection overlaps the outlined main object at IoU 0.5. Named: it also has the human class. $^\dagger$Made the outlines and reference boxes. Best in bold, $^\dagger$ rows aside. Human labels.}
\label{tab:det}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrr}
\toprule
detector & found ($\uparrow$) & named ($\uparrow$) \\
\midrule
Faster R-CNN & 94.2 & 59.8 \\
RetinaNet & 96.6 & 59.9 \\
FCOS & 96.4 & 58.9 \\
YOLO11-m & 97.5 & \textbf{63.4} \\
Faster R-CNN (agreed boxes) & 89.5 & 30.6 \\
Grounding DINO (zero-shot) & \textbf{99.2} & 13.2 \\
OWLv2 (zero-shot)$^\dagger$ & 99.1 & 24.6 \\
SAM~3 (zero-shot)$^\dagger$ & 95.9 & 33.1 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

